Singularity-free Aerial Deformation by Two-dimensional Multilinked Aerial Robot with 1-DoF Vectorable Propeller

Two-dimensional multilinked structures can benefit aerial robots in both maneuvering and manipulation because of their deformation ability. However, certain types of singular forms must be avoided during deformation. Hence, an additional 1 Degrees-of-Freedom (DoF) vectorable propeller is employed in this work to overcome singular forms by properly changing the thrust direction. In this paper, we first extend modeling and control methods from our previous works for an under-actuated model whose thrust forces are not unidirectional. We then propose a planning method for the vectoring angles to solve the singularity by maximizing the controllability under arbitrary robot forms. Finally, we demonstrate the feasibility of the proposed methods by experiments where a quad-type model is used to perform trajectory tracking under challenging forms, such as a line-shape form, and the deformation passing these challenging forms.

==> Makefile <==
# Makefile tips: http://www.ie.u-ryukyu.ac.jp/~e085739/c.makefile.tuts.html

LATEX=platex
MAKEINDEX=makeindex
BIBTEX=pbibtex
LABPAT="^LaTeX Warning: Label(s) may have changed\."
FIGDIR = figs

PDFOPEN = gnome-open

THISDIR = 2021_RAL_ICRA_Hydrus_XI
BASE1=main
CLS=ieeetran.cls
SRCS=main.tex

bases = $(BASE1)
targets = $(bases:%=%.pdf) # http://www.ne.jp/asahi/hishidama/home/tech/unix/cmd/make2.html
bbls = $(bases:%=%.bbl)
#$(warning bbls = $(bbls))

.SUFFIXES: .txt .tex .bbl .bb .jpg .JPG .png .PNG .bmp .BMP .pdf

.jpg.bb:
	@(ebb -b $< 2>/dev/null;)

.JPG.bb:
	@(ebb -b $< 2>/dev/null;)

.png.bb:
	@(ebb -b $< 2>/dev/null;)

.PNG.bb:
	@(ebb -b $< 2>/dev/null;)

.pdf.bb:
	@(ebb -b $< 2>/dev/null;)

BB_FILES = $(shell find ${FIGDIR} -name "*.jpg" | sed s/jpg/bb/g)
BB_FILES += $(shell find ${FIGDIR} -name "*.JPG" | sed s/JPG/bb/g)
BB_FILES += $(shell find ${FIGDIR} -name "*.png" | sed s/png/bb/g)
BB_FILES += $(shell find ${FIGDIR} -name "*.PNG"| sed s/PNG/bb/g)
BB_FILES += $(shell find ${FIGDIR} -name "*.pdf"| sed s/pdf/bb/g)

#$(warning BB_FILES = $(BB_FILES))

%.pdf: %.dvi
	dvipdfmx -V 6 -p letter $<

%.dvi: %.tex
	$(LATEX) $*
	while grep $(LABPAT) $*.log; do $(LATEX) $<; done

%.bbl: %.bib
	$(LATEX) $*
	$(BIBTEX) $*
	$(LATEX) $*

.PHONY: all clean

all: clean $(targets)

bb: $(BB_FILES)

$(CLS): $(CLSORIG)
	cp $(CLSORIG) $(CLS)

$(BASE1).dvi: bb $(BASE1).bbl $(SRCS) $(CLS)

$(bbls): $(CLS)

clean:	bb_bib_clean
	rm -rf *~ *.log *.dvi *.pdf *.aux *.bbl *.blg *.toc *.flc *.bak *.bmc fig.pbm

bb_bib_clean:
	rm -f $(FIGDIR)/*.bb $(FIGDIR)/*/*.bb
	(cd $(FIGDIR); rm -f *~; rm -f *#)

open:
	${PDFOPEN} $(bases).pdf

